Delay Optimal Joint Scheduling-and-Power-Control for Cognitive Radio Uplinks

An uplink cognitive radio system with a single primary user (PU) and multiple secondary users (SUs) is considered. The SUs have an individual average delay constraint and an aggregate average interference constraint to the PU. If the interference channels between the SUs and the PU are statistically different due to the different physical locations of the SUs, the SUs will experience different delay performances. This is because SUs located closer to the PU transmit with lower power levels. A dynamic scheduling-and-power-allocation policy that uses the dynamic programming, is proposed. The proposed policy can provide the required average delay guarantees to all SUs irrespective of their location as well as protect the PU from harmful interference. The policy is shown to be asymptotically delay optimal in the light traffic regime. Motivated, by the high complexity of the dynamic programming algorithm in the optimal policy we exploit the structure of the problem's solution to present an alternative suboptimal policy. Through simulations we show that in both light and heavy traffic regimes, the delay performance of the suboptimal policy is within $0.3\%$ from the optimal policy and both outperforming existing methods.

==> commands.tex <==
%\documentclass{article}
\usepackage{dsfont}
% Gives \ifthenelse
\usepackage{ifthen}
\usepackage{bm} % To use \bm that makes bold characters under math mode
\usepackage{amsmath}
%\usepackage{mathdots}
% Let us add lengths together (e.g., in \settowidth below)
\usepackage{calc}

% Give us commands two two optional arguments
\usepackage{twoopt}

%% Citations use natbib (compare to biblatex below)

% Citations: Numbered (e.g., [1]); Use \citet, \citep, \citeauthor, etc.
%\usepackage[numbers,sort&compress]{natbib}
\usepackage[withbib,all]{authorindex}

%\bibliographystyle{plainnat}
% Tables -- gives us \hline[space] that puts space after \hline
\usepackage{tabls}
% Tables -- gives us horizontal rules that separate columns rather than
% vertical
\usepackage{booktabs}

% Give us nicer listing environments, especially for listing within
% paragraphs. Also adds item labels that can be automatically generated
% and labeled like equations. Compact environments: compactenum and
% compactitem
% (the package enumitem might be a better choice)
\usepackage{paralist}
%\bibliographystyle{abbrvnat}

% Fix referencing of nested enumerations (put a dot between counters)
\makeatletter
\renewcommand{\theenumii}{\arabic{enumii}}
\renewcommand{\labelenumii}{\theenumi.\theenumii}
\renewcommand{\p@enumii}{\theenumi.}
\makeatother

% Mathematical symbols, etc.
\usepackage{amscd,mathrsfs}

%%fakepart{Modern graphics support}
% ---------------------------------------------------------------------|

%% Use subfig for subfigures
%\usepackage[nearskip=-3pt,captionskip=4pt,
%            listofformat=subsimple,labelformat=simple]{subfig}
%\captionsetup[subfloat]{listofindent=4em}
%
%% % Add subfigures to the List of Figures
%% \setcounter{lofdepth}{2}
%
%% Make sure subfigures have parentheses around them everywhere
%\renewcommand\thesubfigure{(\alph{subfigure})}

\usepackage{subfigure}

% Use graphicx for including graphics
\usepackage{graphicx}

\usepackage{hyperref}
% Use pict2e for more advanced picture environment support
\usepackage{pict2e}
%\usepackage{caption}
\usepackage{amsmath}
\usepackage{bbm}
\usepackage{graphicx}
\usepackage{epsfig}
\usepackage{array}
\usepackage{psfrag}
\usepackage{amssymb}
\usepackage{mathdots}
\usepackage{color}
\usepackage{pstricks,pst-node,pst-text,pst-3d,pst-plot}
\usepackage{psfrag}
\usepackage{enumerate}
\usepackage{url,cite}
\usepackage{appendix}
\usepackage{amsfonts}%
\usepackage{amsthm}
\usepackage{dsfont}%
\usepackage{verbatim}%
\usepackage{setspace}
\usepackage{float}
%\usepackage{mathtools} %\triangleq
\usepackage{url}
\usepackage{fancyhdr}
%\usepackage{lipsum} %\footnote
%\usepackage[yyyymmdd,hhmmss]{datetime}
%\rfoot{Compiled on \today}
%\usepackage[toc,page]{appendix}
%\usepackage{fullpage}
%\doublespacing
\usepackage[hmargin=0.6in , vmargin=1in]{geometry}
\usepackage{algorithm}
\usepackage{algorithmic}
\pdfoptionpdfminorversion=6
\newtheorem{thm}{Theorem}
\newtheorem{lma}{Lemma}
%\renewenvironment{proof}{\par{\noindent \it Proof:}}
%\newtheorem{prf}{\par{\noindent \it Proof:}}{\qed\par}
\newenvironment{proofsketch}{\par{\it Proof Sketch:}}{\qed\par}
\newcommand{\gammath}[1]{\gamma_{\rm th}\left( #1 \right)}
\newcommand{\gammathst}[1]{\gamma_{\rm th}^*\left( #1 \right)}
\newcommand{\bfGamma}{{\bf \Gamma}_{\rm th}}
\newcommand{\Gammast}[1]{\bfGamma^{\rm *} \lb #1 \rb}
%\newcommand{\PF}{P^{\rm F}}
%\newcommand{\PFSt}{P^{\rm F *}}
%\newcommand{\PB}{P^{\rm B}}
%\newcommand{\PBSt}{P^{\rm B *}}
\newcommand{\bfP}[1]{{\bf P}_{#1}}
\newcommand{\Pst}[1]{{\bf P}_{#1}^*}
%\newcommand{\PH}{P^{\rm H}}
%\newcommand{\PHSt}{P^{\rm H *}}
\newcommand{\dgamdlamp}[1]{\frac{\partial \gammathst{#1}}{\partial \lambdapst}}
\newcommand{\dUdlamp}[1]{\frac{\partial U_{#1}^*}{\partial \lambdapst}}
\newcommand{\dSdlamp}[1]{\frac{\partial S_{#1}^*}{\partial \lambdapst}}
\newcommand{\dpdlamp}[1]{\frac{\partial p_{#1}^*}{\partial \lambdapst}}
\newcommand{\dgamdlamd}[1]{\frac{\partial \gammathst{#1}}{\partial \lambdadst}}
\newcommand{\dUdlamd}[1]{\frac{\partial U_{#1}^*}{\partial \lambdadst}}
\newcommand{\dSdlamd}[1]{\frac{\partial S_{#1}^*}{\partial \lambdadst}}
\newcommand{\dpdlamd}[1]{\frac{\partial p_{#1}^*}{\partial \lambdadst}}
\newcommand{\dUSpdlamp}[1]{\dUdlamp{#1} - \lambdap \dSdlamp{#1} + \lambdad \dpdlamp{#1}}
\newcommand{\dgamdlami}[1]{\frac{\partial \gammathst{#1}}{\partial \lambdaist}}
\newcommand{\dUdlami}[1]{\frac{\partial \Usoftst_{#1}}{\partial \lambdaist}}
\newcommand{\dIdlami}[1]{\frac{\partial \Isoftst_{#1}}{\partial \lambdaist}}
\newcommand{\dpdlami}[1]{\frac{\partial \psoftst_{#1}}{\partial \lambdaist}}
\newcommand{\dgamdlamdlev}[1]{\frac{\partial \gammathst{#1}}{\partial \lambdadst}}
\newcommand{\dUdlamdlev}[1]{\frac{\partial U_{#1}(\Gammast{#1},P)}{\partial \lambdadst}}
\newcommand{\dpdlamdlev}[1]{\frac{\partial p_{#1}(\Gammast{#1})}{\partial \lambdadst}}
\newcommand{\Pist}[1]{P_{#1}^* \lb \gammathst{#1} \rb}
\newcommand{\pdf}{f_{\gamma}}
\newcommand{\ccdf}{\bar{F}_{\gamma}}
\newcommand{\lb}{\left (}
\newcommand{\rb}{\right )}
\newcommand{\script}[1]{{\mathcal {#1}}}
\newcommand{\prbz}[1]{{\rm Pr} \left[ b_{#1}=1 \vert z \right]}
\newcommand{\fzb}{f_{z \vert b} \lb z \vert b_i=1 \rb}
\newcommand{\fzf}{f_{z \vert b} \lb z \vert b_i=0 \rb}
\newcommand{\Ibessel}[1]{I_{#1}^{\rm Bes}}
\newcommand{\intinf}{\int_{-\infty}^{\infty}}

%Constants:
\newcommand{\Pavg}{P_{\rm avg}}
\newcommand{\Iavg}{I_{\rm avg}}
\newcommand{\rmin}{r_{\rm min}}
\newcommand{\pframe}{P_{\rm frame}}
\newcommand{\Dmax}{\bar{D}_{\rm max}}
\newcommand{\invDmaxline}{1/\Dmax}
\newcommand{\invDmax}{\frac{1}{\Dmax}}
\newcommand{\zb}{z_{\rm b}}
\newcommand{\zf}{z_{\rm f}}
\newcommand{\zth}{z_{\rm th}}
\newcommand{\pmd}{P_{\rm MD}}
\newcommand{\pfa}{P_{\rm FA}}
\newcommand{\pskip}[1]{p_{#1}^{\rm skip}}
\newcommand{\Utwomax}{U_2^{\rm max}}
\newcommand{\ptwomax}{p_2^{\rm max}}
\newcommand{\Ts}{T_{\rm s}}
\newcommand{\ones}[1]{{\bf 1}_{#1}}
\newcommand{\prskip}{p_{\rm skip}}

%Equations:
\newcommand{\pstDmaxline}{p_1^*=\invDmaxline}
\newcommand{\pstDmax}{p_1^*=\invDmax}
\newcommand{\tinset}{t \in \{1,...t_f\}}

% Defining \lambda's
\newcommand{\lambdad}{\lambda_{\rm D}}
\newcommand{\lambdadst}{\lambda_{\rm D}^*}
\newcommand{\lambdap}{\lambda_{\rm P}}
\newcommand{\lambdapst}{\lambda_{\rm P}^*}
\newcommand{\lambdapmin}{\lambdap^{\rm min}}
\newcommand{\lambdapmax}{\lambdap^{\rm max}}
\newcommand{\lambdadmax}{\lambdad^{\rm max}}
\newcommand{\lambdaiz}{\lambdai \prbz}
\newcommand{\lambdaizst}{\lambdaist \prbz}
\newcommand{\Pmax}{P_{\rm max}}


%%%%%%%%%% Overlay parameters:

\newcommand{\Ierr}[1]{I_{#1}^{\rm Err} \lb \Gammast{#1},\Pst{#1} \rb}
\newcommand{\Uerr}[1]{U_{#1}^{\rm Err} \lb \Gammast{#1},\Pst{#1} \rb}

%%%%%%%%%% SOFT Underlay parameters:
% lambda:
\newcommand{\lambdai}{\lambda_{\rm I}}
\newcommand{\lambdaPS}{\lambda_{\rm P}}
\newcommand{\lambdaist}{\lambda_{\rm I}^*}
\newcommand{\lambdaPSSt}{\lambda_{\rm P}^{\rm S *}}
% Power
\newcommand{\PS}[1]{P_{#1}\lb \gamma \rb}
\newcommand{\PSst}[1]{P^*_{#1}\lb \gamma \rb}
\newcommand{\bfPS}[1]{{\bf P}_{#1}}
\newcommand{\bfPSst}{{\bf P}^*}
% \gammaS
\newcommand{\gammaz}[1]{\gamma_{\rm th} \left(#1,z \right)}
\newcommand{\gammazst}[1]{\gamma_{\rm th}^* \left(#1,z \right)}
\newcommand{\GammaS}[1]{\bfGamma \lb #1,z\rb}
\newcommand{\Gammasst}[1]{\bfGamma^{\rm *} \lb #1,z\rb}
% U, S, p and I:
\newcommand{\Usoft}{U}
\newcommand{\Ssoft}{S}
\newcommand{\psoft}{p}
\newcommand{\Isoft}{I}
\newcommand{\Usoftst}{U^*}
\newcommand{\Ssoftst}{S^*}
\newcommand{\psoftst}{p^*}
\newcommand{\Isoftst}{I^*}

\newcommand{\figures}{C:/Users/ewaisha/Desktop/Dropbox/ASU/Research/Latex/HFramedInstInterfHeteroCR/figures}

%%%%%%%%%%%%% Journal 2 Parameters: %%%%%%%%%%%%%%%%%%%%%%
\newtheorem{Def}{Definition}
\DeclareMathOperator{\E}{\mathbb{E}}
%\renewenvironment{proof}{\par{\noindent \it Proof:}}
%\newtheorem{prf}{\par{\noindent \it Proof:}}{\qed\par}
\newcommand{\bP}{\bar{P}}
%\newcommand{\PH}{P^{\rm H}}
%\newcommand{\PHSt}{P^{\rm H *}}
%Constants:
\newcommand{\Pmin}{P_{\rm min}}
\newcommand{\bfpi}{{\bf \pi}}
\newcommand{\Iinst}{I_{\rm inst}}
\newcommand{\fgammai}{f_{\gamma_i}}
\newcommand{\fgi}{f_{g_i}}
%\DeclareMathOperator*{\E}{\mathbb{E}}
\newcommand{\EE}[1]{\E \left[ #1 \right]}
\newcommand{\EEC}[1]{\E_{\bfY(k)} \left[ #1 \right]}
\newcommand{\bgi}{\bar{g}_i}
\newcommand{\bW}{\bar{W}}
\newcommand{\bfW}{{\bf \bW}}
\newcommand{\SA}{A_{\rm S}}
\newcommand{\bfPst}{{\bf P}^*}
\newcommand{\bfS}{{\bf S}}
\newcommand{\bfpist}{{\bm{\pi}}^*}
\newcommand{\bI}{{\bf I}}
\newcommand{\bgamma}{\bar{\gamma}}
\newcommand{\bfg}{{\bf g}}
\newcommand{\bfQ}{{\bf Q}}
\newcommand{\WTA}{W^{\rm TA}}
\newcommand{\ITA}{I^{\rm TA}}
\newcommand{\Xvq}{\{X(k)\}_{k=0}^\infty}
\newcommand{\Yivq}{\{Y_i(k)\}_{k=0}^\infty}
\newcommand{\seq}[1]{\{#1\}_{k=1}^\infty}
\newcommand{\bfY}{{\bf Y}}
\newcommand{\threevec}{$\bfQ(t)$, $\bfGamma^{(t)}$ and $\bfg^{(t)}$}
\newcommand{\bfPsi}{{\bf \Psi}}
\newcommand{\Bw}{B_{\rm w}}
\newcommand{\pardef}[1]{\triangleq [#1_1^{(t)},\cdots,#1_N^{(t)}]^T}
\newcommand{\parFdef}[1]{\triangleq [#1_1(k),\cdots,#1_N(k)]^T}
\newcommand{\DOIC}{\emph{DOIC}}
\newcommand{\DOAC}{\emph{DOAC}}
\newcommand{\Twolev}{\emph{TwoLev}}
\newcommand{\DOACopt}{\emph{DOAC-Pow-Alloc}}
\newcommand{\brho}{\bar{\rho}}
\newcommand{\Ri}{R_i}
\newcommand{\FDurK}{\vert \script{F}_k\vert}
\newcommand{\Wup}{W^{\rm up}_{\pi_i}}
\newcommand{\Wpi}{W_{\pi_i}}
\newcommand{\gammaerr}{\gamma_i^{\rm err}(t)}
\newcommand{\gerr}{g_i^{\rm err}(t)}
\newcommand{\dOne}{29}
\newcommand{\dTwo}{40}
\newcommand{\Obj}{O_{\rm obj}}
\newcommand{\trho}{\tilde{\rho}}
\newcommand{\tS}{{\bf \tilde{S}}}
\newcommand{\sS}{\script{S}}

%\renewenvironment{proof}{\par{\noindent \it Proof:}}
%\newtheorem{prf}{\par{\noindent \it Proof:}}{\qed\par}
%\newenvironment{proofsketch}{\par{\it Proof Sketch:}}{\qed\par}
%\newcommand{\gammath}[1]{\gamma_{\rm th}\left( #1 \right)}
%\newcommand{\gammathst}[1]{\gamma_{\rm th}^*\left( #1 \right)}
%\newcommand{\Gammast}[1]{\bfGamma^{\rm *} \lb #1 \rb}
%\newcommand{\PF}{P^{\rm F}}
%\newcommand{\PFSt}{P^{\rm F *}}
%\newcommand{\PB}{P^{\rm B}}
%\newcommand{\PBSt}{P^{\rm B *}}
%\newcommand{\bP}{\overline{P}}
%\newcommand{\Pst}[1]{{\bf P}_{#1}^*}
%\newcommand{\PH}{P^{\rm H}}
%\newcommand{\PHSt}{P^{\rm H *}}
%\newcommand{\Pist}[1]{P_{#1}^* \lb \gammathst{#1} \rb}
\newcommand{\cdf}{F_{g_{\pi_j}}}
%\newcommand{\lb}{\left (}
%\newcommand{\rb}{\right )}
%\newcommand{\prbz}[1]{{\rm Pr} \left[ b_{#1}=1 \vert z \right]}
%\newcommand{\fzb}{f_{z \vert b} \lb z \vert b_i=1 \rb}
%\newcommand{\fzf}{f_{z \vert b} \lb z \vert b_i=0 \rb}
%\newcommand{\Ibessel}[1]{I_{#1}^{\rm Bes}}
%\newcommand{\intinf}{\int_{-\infty}^{\infty}}

%Constants:
%\newcommand{\script}[1]{{\mathcal {#1}}}
%\newcommand{\Pavg}{P_{\rm avg}}
%\newcommand{\Pmax}{P_{\rm max}}
%\newcommand{\Pmin}{P_{\rm min}}
\newcommand{\Pminn}{P^{\rm min}}
%\newcommand{\Iinst}{I_{\rm inst}}
%\newcommand{\Iavg}{I_{\rm avg}}
\newcommand{\gmax}{g_{\rm max}}
%\newcommand{\fgammai}{f_{\gamma_i}}
%\newcommand{\fgi}{f_{g_i}}
%\DeclareMathOperator*{\E}{\mathbb{E}}
%\newcommand{\EE}[1]{\E \left[ #1 \right]}
\newcommand{\EEU}[1]{\E_{\bfU(k)} \left[ #1 \right]}
\newcommand{\EEY}[1]{\E_{\bfY(k)} \left[ #1 \right]}
\newcommand{\Prob}[1]{{\bf Pr}\left[ #1 \right]}
%\newcommand{\bgi}{\overline{g}_i}
%\newcommand{\bW}{\overline{W}}
%\newcommand{\bfW}{{\bf \bW}}
%\newcommand{\SA}{A_{\rm S}}
\newcommand{\Pit}{P_i^{(t)}}
\newcommand{\git}{g_i^{(t)}}
%\newcommand{\bfP}{{\bf P}}
%\newcommand{\bfPst}{{\bf P}^*}
%\newcommand{\bfS}{{\bf S}}
%\newcommand{\bfpi}{{\bm{\pi}}}
%\newcommand{\bfpist}{{\bm{\pi}}^*}
%\newcommand{\bI}{{\bf I}}
%\newcommand{\bfGamma}{{\bf \Gamma}}
%\newcommand{\bgamma}{\overline{\gamma}}
%\newcommand{\bfg}{{\bf g}}
%\newcommand{\bfQ}{{\bf Q}}
%\newcommand{\WTA}{W^{\rm TA}}
%\newcommand{\ITA}{I^{\rm TA}}
%\newcommand{\Xvq}{\{X(k)\}_{k=0}^\infty}
%\newcommand{\Yivq}{\{Y_i(k)\}_{k=0}^\infty}
%\newcommand{\seq}[1]{\{#1\}_{k=0}^\infty}
%\newcommand{\bfY}{{\bf Y}}
\newcommand{\bfU}{{\bf U}}
\newcommand{\bfr}{{\bf r}}
%\newcommand{\threevec}{$\bfQ(t)$, $\bfGamma^{(t)}$ and $\bfg^{(t)}$}
%\newcommand{\bfPsi}{{\bf \psi}}
%\newcommand{\Bw}{B_{\rm w}}
%\newcommand{\pardef}[1]{\triangleq [#1_1^{(t)},\cdots,#1_N^{(t)}]^T}
%\newcommand{\parFdef}[1]{\triangleq [#1_1(k),\cdots,#1_N(k)]^T}
\newcommand{\mui}{\EE{\Ri}}
\newcommand{\psiI}{\psi_{\pi_j}^{\rm I}}
\newcommand{\psiD}{\psi_{\pi_j}^{\rm D}}
\newcommand{\psiInt}{\psi^{\rm I}}
\newcommand{\psiDel}{\psi^{\rm D}}
\newcommand{\mupiP}{\mu_{\pi_j}(P)}
\newcommand{\DbyDP}[1]{\frac{\partial #1}{\partial P}}
\newcommand{\gammait}{\gamma_i^{(t)}}
\newcommand{\tP}{\tilde{P}}
\newcommand{\tPsi}{\tilde{\Psi}}
\newcommand{\chiDOAC}{\chi^{\rm {\DOAC}}}
\newcommand{\BW}{B_{\rm W}}
\newcommand{\brhomax}{\brho^{\rm max}}
\newcommand{\brhomin}{\brho^{\rm min}}
\newcommand{\sB}{\tau^{\rm B}}
\newcommand{\sNB}{\tau^{\rm NB}}
\newcommand{\Prho}{P_{\rho}\lb \pi_j,\brho_{\pi_N}\rb}
\newcommand{\psirho}{\Psi_{\rho}\lb\brho_{\pi_N}\rb}
\newcommand{\Prhost}{P_{\rho}\lb \pi_j,\rho^*\rb}
\newcommand{\psirhost}{\Psi_{\rho}\lb\rho^*\rb}
\newcommand{\bflambda}{{\bf \lambda}}
\newcommand{\gammamini}{\gamma_i^{\rm min}}

%\newcommand{\Ts}{T}
%\newcommand{\ones}[1]{{\bf 1}_{#1}}
\newcommand{\HOL}{L^{\rm rem}}
\newcommand{\widthn}{0.8}
\newcommand{\Rmax}{R_{\rm max}}
\newcommand{\gammamax}{\gamma_{\rm max}}
\newcommand{\DF}{D_{\rm F}}
